Reconfigurable Heterogeneous Quorum Systems

In contrast to proof-of-work replication, Byzantine quorum systems maintain consistency across replicas with higher throughput modest energy consumption, and deterministic liveness guarantees. If complemented with heterogeneous trust and open membership, they have the potential to serve as blockchains backbone. This paper presents a general model of heterogeneous quorum systems where each participant can declare its own quorums, and captures the consistency, availability and inclusion properties of these systems. In order to support open membership, it then presents reconfiguration protocols for heterogeneous quorum systems including joining and leaving of a process, and adding and removing of a quorum, and further, proves their correctness in the face of Byzantine attacks. The design of the protocols is informed by the trade-offs that the paper proves for the properties that reconfigurations can preserve. The paper further presents a graph characterization of heterogeneous quorum systems, and its application for reconfiguration optimization.

==> LeaderElection.tex <==
\newpageprime
% \subsection{\textbf{Leader Election}}
\subsection{Leader Election}

☞{The proof variable in the protocol ... }

We use sink discovery protocol to construct a eventual leader election module.
The insight is after the sink discovery protocol, $\ProtoSink$ is a fixed set of well-behaved processes.
They are strongly connected despite Byzantine failures in the system.
They can communicate with each other and collect the process identities with a vaild proof for $\insink$ variables.
Then based on a pre-defined order across all processes (for instance, smallest process identity), 
exponential timeout back-off and 
a round-robin leader election approach to exclude the Byzantine processes,
eventually all the processes in $\ProtoSink$ elect the same well-behaved leader.
Finally, they propagate elected leader to their followers to finish the leader election process.

\begin{algorithm}
	\caption{Eventual Leader Election}
	\label{alg:leaderelection}
	\DontPrintSemicolon
	\SetKwBlock{When}{when received}{end}
	\SetKwBlock{Upon}{upon}{end}
	\Implements $\colon$ \ $\LeaderProto$\;
	%\ \ \ $\request : \Leave$ \;
	\ \ \ $\response : \Elect(p)$
	
	\textbf{Variables:}   \;
	\ \ \ $Q$ \Comment{The individual minimal quorums of $\self$} \;
	\ \ \ $\insink : \mathsf{Boolean}$ \;
	\ \ \ $F : 𝓟$ \;
	\ \ \ $\proofLE : \mathsf{Set}[\text{Exchange or Extend messages}]$\;	
	\ \ \ $\sink : \mathsf{Set}[𝓟]$ \;
	
	\Upon ($\insink = \true$){  
		$\request \ \apl(p), \Propagate(\self, \proofLE)$ \mbox{ for each} $p ∈ \cup Q$ \label{algLE:sendproof}
	}
	
	\Upon ($\response$ \mbox{$\apl (p)$}, \mbox{$\Propagate(p', \proofLE')$} ){
		\If{$\proofLE'$ is valid}{
			$\sink \leftarrow \sink \cup \{p'\}$ \;
			$\request \ \apl(p''), \Propagate(p', \proofLE')$ \mbox{ for each} $p'' ∈ \cup Q$\label{algLE:passproof} \;
		}
	}
	
	\Upon (After GST){  
		\If{$\insink = \true$}{
			$\response \ \Elect(p)$ such that $p \in \sink$ and is choosen based on pre-defined order \label{algLE:election1} \;
			$\request \ \apl(p'), \PropagateF(p, Q)$ \mbox{ for each} $p' ∈ F$ \label{algLE:passF}\;
		}
	}

	\Upon ($\response$ $\overline{\mbox{$\apl(p)$}}$, \mbox{$\PropagateF(p', Q')$} from each $p \in q$ s.t. $q \in Q' \wedge \textcolor{blue}{Validate(q)}$ \label{algLE:receiveQ}){  
		$\response \ \Elect(p')$ \label{algLE:election2}\;
	}
	
\end{algorithm}

Each well-behaved process keeps the following local variables for leader election:
$\Q$ stores the individual minimal quorums for $\self$, which can be different for distinct well-behaved processes.
$\insink$ is a boolean variable indicates whether $\self$ is in the sink component of the quorum graph.
$\proofLE$ is a set of $\Exchange$ or $\Extend$ messages that serves as a proof when $\insink$ is set to $\true$.
They are set by the sink discovery protocol.
$F$ is the follower set for $\self$ which stores a set of processes that consult $\self$ for consensus.
$\sink$ is a set of processes that are verified to be in the sink component of quorum graph.
Notice that $\sink$ variables are updated gradually and we only ensure that they eventually converge to the same value for all the well-behaved processes.


\begin{lemma}
	Eventual leader election protocol has eventual agreement: There is a time after which no two well-behaved processes trust different processes.
\end{lemma}

There are two cases where leader $p$ is elected by a well-behaved process. We prove agreement for both cases.
In the first case, leader is elected by a process in $\ProtoSink$ at \autoref{algLE:election1}.
Eventually all the processes in $\ProtoSink$ have the same $\sink$ variable by the epidemic $\Propagate$ messages they send to each other.
Then based on a pre-defined order across all processes, they will elect the same leader.

In the second case, leader is elected by a process out of $\ProtoSink$ at \autoref{algLE:election2}.
A well-behaved process only elects a leader if it receives $\PropagateF$ messages from a minimal quorum $q$ with at least one well-behaved member.
By quorum consistency, the elected leaders are the same for all the well-behaved processes.


\begin{lemma}
	Eventual accuracy: There is a time after which every well-behaved process with weak availability
	trusts some well-behaved process.
\end{lemma}

Each process keeps a local variable to store the processes in $\ProtoSink$ in $\sink$.
By the definition of strongly connected component and \autoref{lem:acc-1} and \autoref{lem:acc-2}, $\ProtoSink \subseteq \Sink$ and can reach all the well-behaved processes in $\Sink$.
$p \in \ProtoSink$ sends out their identity and a valid proof to all the processes in their quorums at \autoref{algLE:sendproof}.
Any process receives the $\Propagate$ message verify the correctness of the proof and update $\sink$ variable. 
They also propagate the process identity they received and the proof to their quorum members at \autoref{algLE:passproof}.
After the global stabalization time, all the well-behaved processes in $\Sink$ will have the same $\sink$ variable and elect the same leader based on the pre-defined order at \autoref{algLE:election1}.
By \autoref{lem:lemma2}, every the well-behaved process with weak availability is the follower of a well-behaved minimal quorum.
By \autoref{lem:exchange_complete}, they will eventually receive the propagation message send at \autoref{algLE:passF} from the well-behaved minimal quorum.
%at \autoref{algLE:receiveQ}.
Then they elect the leader at $\autoref{algLE:election2}$.



\begin{comment}
	\textbf{∗Preservation of quorum intersection. \ }
	
	By \autoref{lem:outlive-min-inter},
	at the beginning of execution,
	every outlive heterogeneous quorum system
	has
	outlive minimal quorum intersection.
	% 
	% \begin{lemma}
		% \label{lem:exec-leave-min-inter}
		% Every 
		% execution of
		% an outlive quorum system that 
		If the reconfiguration protocols of the system
		preserve outlive minimal quorum intersection
		% with the $\Leave$ protocol
		then
		the whole execution 
		enjoys
		outlive minimal quorum intersection.
		% \end{lemma}
	% 
	% And then for inductive steps
	% by \autoref{lem:leave-pres-inter}.
	% 
	% 
	% 
	% \begin{lemma}
		% \label{lem:exec-leave-inter}
		% 
		% By \autoref{lem:exec-leave-min-inter} and 
		Further, 
		by \autoref{lem:lemma0},
		and the fact that 
		having an intersection with the outlive set is a superset-closed property,
		we have that
		every execution
		% every 
		% execution of
		% an outlive quorum system 
		% with the $\Leave$ protocol
		enjoys
		outlive quorum intersection,
		% \end{lemma}
	% 
	% 
	that by \autoref{lem:q-inter-inter}
	immediately implies quorum intersection.
	
	% \begin{lemma}
		% \label{lem:exec-leave-inter-final}
		% Every 
		% execution of
		% an outlive quorum system with
		% the $\Leave$ protocol
		% enjoys
		% quorum intersection.
		% \end{lemma}
	% 
	% By \autoref{lem:exec-leave-inter}
	% and
	% \autoref{lem:q-inter-inter}.
	
	In the following sections,
	we prove that 
	each reconfiguration protocol
	preserve outlive minimal quorum intersection.
\end{comment}

% ☞{Merge with the original definitions.}


==> Measurements.tex <==
% \section{Stellar Network Measurements}
% \section{Possibility of Reconfiguration Attacks}
\section{Reconfiguration Frequency and Possibility of Attacks}
\label{sec:reconfig-attack}
% \section{Openness and Reconfiguration Attacks}


% \xl{Explain why we choose stellar as the example for potential attacks: stellar and its family of blockchains are the only real world blockchain applications that enable heterogeneous trusts. We motivate the paper with measurements from stellar since it is the most decentralized and practical one in HQS setting.}

% \begin{wrapfigure}{R}{0.32\textwidth}
\begin{figure}
%\vspace{-3ex}
\small
\includegraphics[width=0.5\linewidth]{all_arrive_leave.pdf}\includegraphics[width=0.5\linewidth]{all_cumulative.pdf}

(a) Network Churn for 90 Days
(b) Cumulative Network Churn

\includegraphics[width=0.5\linewidth]{response_time.pdf}\includegraphics[width=0.5\linewidth]{peer_latency_stacked.pdf}

(c) Transaction Response Time
(d) Communication Latency

\caption{Network Churn and Latency}
\label{fig:measurements}
% \end{figure*}
% \end{figure*}
% \vspace{-1.5ex}
%\vspace{-2ex}
\end{figure}


Stellar operates a global ledger system with a heterogeneous quorum system.
%
% the need for safe reconfiguration protocols is further noticed.
% felt
% becomes evident.
% 
In this section, we present 
network churn and delay
measurements for the real-world Stellar network.
% to gauge the possibility of reconfiguration attacks.
% and present potential reconfiguration attacks. 
The measurements suggest that the Stellar network experiences a high churn,
increasing the likelihood of reconfiguration attacks,
and that its network latency can be high enough 
to leave a time window for potential attacks
that we describe.
%
% 
Stellar enforces a hierarchy for its quorums to have quorum intersection,
and avoid reconfiguration attacks.
As the Stellar network grows larger and allows more decentralized configurations,
the need for safe reconfiguration protocols is further emerging
\cite{saad2022three,saad2021syncattack}.
In the next sections, we present reconfiguration protocols 
that can be used to prevent these attacks.
% that the Stellar network can use to prevent these attacks.
% 
% For measurements, we leveraged the APIs provided by the online service stellarbeats.io \cite{stellarbeat}, and Stellar's own horizon services.
% Stellarbeat connects to nodes in the Stellar public network, and captures SCP messages to verify whether a node is actively participating in the Stellar consensus protocol.

% (1) the network delay in the real world
% (2) the network churn caused by the open nature of HQS, and
% (3) partitioning possibility due to the churn.



% \subsection{Stellar Network Churn}
\textbf{Network Churn. \ }
% 
Each node on the Stellar network has a public key that it uses to sign transactions.
% attack vulnerability can be potentially exploit, 
We used
the online service stellarbeats.io \cite{stellarbeat}
to record the public keys,
and analyzed how frequent reconfigurations are.
% measure the network churn by
% for both all the nodes and only validator nodes.
% 
% 
% Let the set of nodes in day $i$ be $S_{i}$.
% Then the arriving nodes for day $i$ is $S_{i} \setminus S_{i-1}$.
% Similarly, the departing nodes for day $i$ is $S_{i-1} \setminus S_{i}$.
In \autoref{fig:measurements}.(a)
% graph \ref{fig:arrive_leave_all} and \ref{fig:arrive_leave_validator}, 
we show the number of arriving and departing nodes per day for three months:
% We collected Stellar network data from 
Feb 1 to May 1, 2023.
% for churn measurements.
% 
The results shows that on average 7\% of nodes arrive at and depart from the network every day.
The maximum number of nodes arriving or departing on a single day is 59, which is close to 40\% of the network size.
% 
In \autoref{fig:measurements}.(b),
% In graph \ref{fig:cumulative_all} and \ref{fig:cumulative_validtors} 
we show the number of nodes that were present in the system in each day of the month, 
and the cumulative number of nodes that ever appeared in the network until that day.
This graph shows that although 
the network maintains a stable size,
it experiences notable churn.
%
(We obtained similar results for the churn of validator nodes that we report 
at the end of this section.)
% in the appendix 
% \autoref{sec:measurements-app}.)




% \subsection{Stellar Network Synchronization}
\textbf{Network Delay. \ }
% 
% 1.
% ☞{Transaction response time: 5 seconds}
To estimate transaction response time,
we obtained data using the Horizon API \cite{horizonapi}.
It reports the ledger close time
which is the duration from the time a transaction is submitted to the time when it appears on the chain.
We collected ledger close times for 200 ledgers (the maximum number of ledgers that can be retrieved one time), five times during a day (1000 datapoints).
\autoref{fig:measurements}.(c) shows the distribution of ledger close time.
Horizon API reports this time in discrete seconds.
The average is 5.75 seconds. 
% and remains stable.


% 2.
To measure the latency of communication between peers,
we used the stellar-core API \cite{stellarcore}.
% and horizon API
% Although the stellar-core API is often private,
% to the stellar node itself, 
We were able to connect to 
% only 
three geo-distributed nodes in three areas:
Hong Kong, Finland and Germany.
We measured the communication latency between each node and its peers.
These nodes are connected to 30 validators (which is about half of the network's validators).
We collected the communication latency for 10 minutes 5 times during a day (27000 datapoints).
% (The servers refused to respond to more requests.)
\autoref{fig:measurements}.(d) shows the cumulative distribution of the latency.
%The average is ☞{5.?} seconds with the large variance of ☞{?}.
Up to 16.8\%, 21.8\% and 15.2\% of the collected latencies from the three validators are larger than
the average ledger close time (5.75s) that we saw above.
% \xl{Our results are correct. The reviewer is confused with the time units in figure 1 (c) and (d)}


% 3.
%☞{Better name: Staleness, or delay}
%
In order to prevent network forks, processes perform an intersection check upon any change in their own quorums.
(The intersection check is proved to be NP-hard even when all the quorum information in the system is available \cite{lachowski2019complexity}, \cite{gaul2019mathematical}.)
% 
To measure the staleness of the intersection check,
we use the stellar-core and horizon APIs
to measure the difference of 
the latest closed ledger when the node performed the intersection check, and the current latest ledger on the network.
We retrieved data from the same three nodes above.
We collected the difference for 10 minutes 5 times during a day.
The average difference for the three nodes are 11211, 11319 and 11605 blocks respectively.



%☞{Local latest vs. Latest in the whole network, for local ones we calculate the maximum}
%we compare the latest block reported by participants of Stellar consensus
%with 
%the latest block on the blockchain tip of all the nodes.

%When the 
%In graph \xl{graph 1}, we show the percentage of nodes that are not synchronized with the latest block.
%☞{What is the interval?}

%When the network is not synchronized, 
%the nodes that are left behind are vulnerable to the partition attack.
%☞{From synchronization of transactions to delay for reconfiguration.}
%Since the most recent quorum information have not been reflected on their state, 
%they may change their own quorum in the meanwhile and sabotage quorum intersection unintentionally.
%☞{They are not aware of other quorums that may have been added.}

%In graph \xl{graph 2}, we show the largest block difference on the Stellar network, which indicate the potential attack window.
%☞{The max difference for all nodes.}




% In Stellar network, there are three types of nodes: watcher nodes, validator nodes and archiver nodes.
% Only validator nodes are responsible to voting for the next block, and can endanger consistency and termination.
% %Therefore, we focus on measuring the churn for validator nodes.
% Each validator node has a public key that is used to sign transactions.
% In order to analyze how frequent the reconfiguration attack vulnerability can be potentially exploit, 
% we measure the network churn by recording the public keys that appear on Stellar network for both all the nodes and only validator nodes.
% For the validator nodes, the number of nodes arriving at and departing from the network is lower.
% However, churn happened in over 15 days out of the 90 day period.

% \input{churn_fig}


\textbf{Potential Reconfiguration Attacks. \ }
% \xl{I do not understand why we need to add $\{1, 3\}$ to $Q(1)$ (reviewer B's comment). We can not assume the newly added quorum ($q_2$) satisfy quorum inclusion since Stellar do not enforce any check for inclusion.}
% \textbf{Potential Attack Scenarios. \ }
% \subsection{Potential Attack Scenario}
% 
Let $\P = \{1, 2, 3, 4 \}$ where the Byzantine set is $\{4\}$.
Let the quorums of process $1$ be $\Q(1) = \{\{1, 2, 4\}\}$.
Similarly, let $\Q(2)  =\{\{1, 2\},$ $\{2, 3\}\}$ and $\Q(3) = \{\{2, 3\}\}$.
(The Byzantine process $4$ can declare arbitrary quorums.)
% as $\Q(4) = \bot$.
This quorum system enjoys quorum intersection for 
% all the 
well-behaved processes 
since all pairs of quorums intersect at a well-behaved process.
% Further, it enjoys quorum availability for processes $2$ and $3$
% % a subset of well-behaved processes 
% since $\{2, 3\}$ is a quorum for both.
% % of its two members.
Let 
% us assume 
the process $2$ add a quorum $q_1= \{2, 4\}$ into $\Q(2)$.
The quorum $q_1$ intersects all the existing quorums at the well-behaved process $2$.
% Let us assume 
Similarly, let 
% another scenario 
the process $3$ add a quorum $q_2 = \{1, 3\}$ into $\Q(3)$.
The quorum $q_2$ intersects all the existing quorums at the well-behaved processes $1$ or $3$.
Both reconfiguration requests seem safe, and if requested concurrently, may be both permitted.
However, the two new quorums do not intersect.
% $q_1 \cap q_2 = \emptyset$.
A user can issue a transaction to spend some credit at process $2$ with $q₁$,
and another transaction to spend the same credit at process $3$ with $q₂$.
That leads to a double-spend and a fork.

After processes $2$ and $3$ add the two quorums, 
they can send updates to other processes.
Then they immediately start executing the double spend transaction.
A successful attack requires
the time to send and receive updates
% about quorum updates
to be larger than
the time to process a transaction.
% 
% To prevent this attack,
% The attack needs
% the time needed for a node to inform other nodes about quorum updates
% to be larger than
% the time to process a transaction.
% the time needed for a node to inform other nodes about quorum updates
% should be less than the time needed to process a transaction.
Considering the measurements above,
this attack is feasible:
the communication delay can be larger than the ledger close time.
%
Interestingly, 
as the network improves its close time,
the attack becomes more feasible.
% 
Similarly, a leave operation can lead to double-spends.
% For example 
In our example, if process $2$ leaves the system, 
quorum intersection is lost.
% In this paper, 
We will present reconfiguration protocols that
constantly preserve quorum intersection;
therefore, they prevent these attacks.
% then the remaining quorums do not intersect at a well-behaved process.

\todo{These attacks 
% can fork 
are feasible in
networks that exhibit high churn and communication delay.
}


% Later any protocol that runs on top of this updated quorum system can violate consistency, including fork in the blockchain.

% Consistency can be violated when the well-behaved process in the intersection of quorums leaves the system without any synchronization.
% For example, if process $2$ in the previous example leaves the system, then the remaining quorums in the system do not intersect at a well-behaved process.
% %☞{Need to Synch between them, need a protocol.}

%☞{This can happen for all four operations not just add.}

%\xl{How to generalize our protocols to the cardinality or dissemination quorum systems?}
%☞{In the protocol section. Necessary?}

%\input{churn_fig}



% \clearpage
\textbf{Extra Measurements. \ }
% \section{Extra Measurements}
\label{sec:measurements-app}
% 
We collected measurements for the churn of validator nodes as well.
The following graphs are similar to the graphs in the main body
except that they report dedicated measurements for the validator nodes.

\includegraphics[width=\linewidth]{validator_arrive_leave}

\includegraphics[width=\linewidth]{validator_cumulative}


==> ResilienDB_GroupMembership.tex <==
\section{Asymmetric Dissemination Quorum Systems}
We generalize the dissemination quorum systems to the our asymmetric trust model. 
A asymmetric byzantine quorum system $\mathbb{Q} = [\mathcal{Q}_1, \mathcal{Q}_2, ..., \mathcal{Q}_n]$, where $\mathcal{Q}_i \subset 2^{\mathcal{P}}, i = [1, n]$. The corresponding asymmetric failure-prone system is $\mathbb{F} = [\mathcal{F}_1, \mathcal{F}_2, ..., \mathcal{F}_n]$. Because we are in a open membership model, a process $p_i$ may not have complete knowledge of the other processes in the system. We use a similar approach to Stellar, process only has the knowledge of its own minimal vertex quorums. The failure prone set for $p_i$ is $\mathcal{U} \setminus \mathcal{Q}_i$. It means that process does not trust any set of nodes which are not its minimal vertex quorums. This definition of fail-prone set is supposed to be complete but may not be accurate. If we define a set of Byzantine processes $B$ for a specific run, then we can guarantee the safety and liveness for a set of processes with the following properties:

%1. AD-safety: For $p_i$, $\exists F_ \in \mathcal{F}_i. B \subseteq F.$

1. AD-consistency and availability: For $p_i, p_j \in U$, $\forall Q_i \in \mathcal{Q}_i, Q_j \in \mathcal{Q}_j, Q_i \cap Q_j \nsubseteq B$ (intertwined).

%2. AD-availability: For all $p_i \in U, \exists Q_i \in \mathcal{Q}_i, Q_i \cap B  = \emptyset$ 

The condition can ensure consistency and availability at the same time if minimal vertex quorums of processes can be changed.
In other words, we extend the totality to all the correct nodes which keep quorum intersection with at least one correct node.

If a befouled node receiving conflicting echo messages and ready messages, how can it distinguish the correct node and Byzantine node? 

When removing nodes, all the minimal vertex nodes need to agree. We assume that Byzantine node always agree a correct node to leave. Because the absence of correct node gives Byzantine nodes more opportunity to manipulate other correct nodes.

Adding quorum or slices can even break quorum intersection.

\section{Byzantine Failure Detector}

It is important to notice that byzantine failure detector is not as easy as perfect failure detector for crash failure. Because the notion of good performance depends on the specific protocol requirements. In this case, we implement the byzantine failure detector for federated voting algorithm. To ensure the accuracy property of the failure detector, we open up the higher-level algorithm and reason about their behaviors.

$\mathit{P}$

$\mathbf{Indication:} \langle bfd, Byzantine | p \rangle: $ Indicates that process $p$ is byzantine.

$\mathbf{Weak \ Completeness:}$ Eventually, every process that exhibit byzantine behavior is permanently detected by every correct process.

$\mathbf{Strong \ Accuracy:}$ If a process $p$ is detected by any correct process, then $p$ had byzantine behavior before the detection.

$\mathbf{Eventual \ Accuracy:}$ Eventually, no correct process is suspected by any correct process.

$\Omega$

Question: how to describe that we can implement reliable broadcast/consensus when there is only partial knowledge about the system? Is there reduction from the algorithm to the minimal knowledge about the system?
%$\mathbf{Eventual \ Accuracy:}$ Eventually, no correct process is suspected by any correct process.

The key point of identifying the byzantine process is similar to leader election: "trust but verify". We notice that only befouled process can be the victim of byzantine behaviors. Because stellar voting guarantees safety and liveness for intact nodes already. Correct but befouled nodes can lose liveness and not deliver any value in order to protect safety. Whenever a process is stuck, which means it receives contradictory ready messages from different senders, it is sure that there is byzantine process inside its own quorum. By removing the byzantine processes from its quorum slices, the befouled process can join the intact set and enjoy safety and liveness. (Do we have false detection? Can we use eventual byzantine failure detector?)

The specifications for byzantine reliable broadcast:

$\mathbf{Validity:}$ If a correct process $p$ broadcast a message m, then it eventually delivers m.

$\mathbf{No duplication:}$ Every correct process delivers at most one message.

$\mathbf{Integrity:}$ If some correct process delivers a message $m$ with sender $p$ and process $p$ is correct, then $m$ was previously broadcast by $p$.

$\mathbf{Agreement:}$ If some correct process delivers a message $m$ then all correct process eventually delivers a message $m$.

In a partially synchronized system with only crash failures, we can implement reliable broadcast without any failure detector. However, we can not implement byzantine reliable broadcast in a partially synchronized system.

The impossibility result: It is not possible to implement byzantine reliable broadcast deterministically for all correct nodes without any byzantine failure detector in the partially synchronous system, even with only one byzantine failure.

%The impossibility result: It is not possible to implement byzantine reliable broadcast deterministically for all correct nodes without a eventual byzantine failure detector in the partially synchronous system.

Proof: We can prove the impossibility result by contradiction. Let's assume that we have an algorithm $\mathcal{A}$ that implements byzantine reliable broadcast in an eventual synchronous system without any failure detector. Then we construct bivalent (or stuck?) admissible initial configuration that does not reach termination. 

%by assuming a byzantine sender. Here the definition of bivalent is not the same as consensus. Because processes does not have initial values. The configuration refers to a vector which records the value broadcast by sender $s$. The potential value can be $m, m', $ or $\bot$, which gives byzantine process $s$ to broadcast contradicting messages to different processes or does not broadcast anything at all.

We first prove that there is a initial configuration that all the admissible run has to reach termination with a byzantine sender. We construct two admissible runs $\mathcal{R}_1, \mathcal{R}_2$. We have the process $s$ broadcast a message $m$. In the initial setting of $\mathcal{R}_1$, we assume $s$ is correct and all the processes are correct. In $\mathcal{R}_2$, all the initial settings are the same except that and $s$ is now faulty and there exists byzantine process. In $\mathcal{R}_1$, according to validity and agreement, all the correct processes delivers $m$ eventually. Let's assume that the first correct process $p$ delivers $m$ at $t'$. Then the run up to time $t'$ is denoted as $\sigma$. The processes who take steps in $\sigma$ is denoted as $S_\sigma$. Then we apply $\sigma$ to $\mathcal{R}_2$ and get the delivery of $m$ in process $p$. Now we assume that $\exists q \in S_\sigma$ and $q$ is Byzantine. According to agreement property, all the other correct process has to deliver $m$ as well.

%We first prove that there is a bivalent initial configuration for any $\mathcal{A}$. Assume not. Then $\mathcal{A}$ must can both deliver $m$ and $m'$ for all correct processes in different initial configurations. When the sender is correct and only broadcast $m$ or $m'$, it is obvious that all the correct processes will deliver $m$ or $m'$ accordingly. We consider the initial configuration where $s$ is byzantine and sends conflicting messages for different processes. 

%Then we construct two admissible runs $\mathcal{R}_1, \mathcal{R}_2$. We have the process $s$ broadcast a message $m$. In the initial setting of $\mathcal{R}_1$, we assume $s$ is correct. In $\mathcal{R}_2$, all the initial settings are the same except that and $s$ is now faulty and only broadcast the message $m$ to $Q_1$ and $m'$ to $Q_2, p \in Q_1 \cap Q_2$. 

%In $\mathcal{R}_1$, according to validity and agreement, all the correct processes delivers $m$ eventually. Let's assume that the first correct process $q$ delivers $m$ at $t'$. We assume that in $\mathcal{R}_1$, there is a process $p$ that does not take any step up to $t'$. $\mathcal{R}_1$ exists. Because if $p$ is byzantine process, it can take no step and according to the validity and agreement, other correct processes have to deliver a message eventually as long as the sender is correct. 

%In $\mathcal{R}_3$, all the prefix up to time $t'$ is the same as $\mathcal{R}_1$. Then $q$ delivers the message $m$ at time $t'$, Since $q$ is a correct process, then all the correct processes have to deliver $m$ eventually, including $p$. 

\section{Group Membership}
At any point in time, the view of the FBQS is $V = ( id, \mathit{S} )$. $id$ is a unique numeric view identifier and $\mathit{S}$ is the quorum slices function. The initial group view is a FBQS $\langle 0, \mathit{S}_0 \rangle$ with quorum intersection property. The group membership abstraction uses indication $\langle View | V \rangle$ to install a new view. We consider a monotone group membership abstraction, where all correct processes install new views in a sequence with monotonically increasing view identifier. When two correct processes install a view with the same identifier, the quorum slices function must be the same.

$\mathbf{Indication:} \langle gm, View | V \rangle: $ Install a new view $V = (id, \mathit{S})$ with view identifier $id$ and quorum slices function $\mathit{S}$.

$\mathbf{Properties}:$

$\mathbf{Monotonicity:}$ If a process $p$ install a view $V = (id, \mathit{S})$ and subsequently another process $q$ install a view $V' = (id', \mathit{S}')$, then $id < id'$.

$\mathbf{Uniform \ Agreement:}$ If some process installs a view $V = (id, \mathit{S})$ and another process install some view $V' = (id, \mathit{S}')$, then $\mathit{S} = \mathit{S}'$.

$\mathbf{Completeness: }$ If a process $p$ is byzantine, then eventually every correct process $q$ install a view $(id, \mathit{S})$ such that $p \notin \mathit{S}(q)$.

$\mathbf{Accuracy:} $ If some process $p$ install a view $(id, \mathit{S})$ with $q \notin \mathit{S}(p)$ for some process $q$, then $q$ is byzantine process.

The scope of underlying consensus component : The top tier? or the quorum is enough?

%\section{BFT with open membership}
%1. At the start of each round, each strongly connected component of the byzantine quorum graph choose a single transaction of a local client. Then they

\section{View-change}

The high level idea is that every time an existing node need to report a suspicion of two different parties which have contradicting opinions. This is because the correct node in the quorum intersection will cast its decision to all the nodes that include itself as minimal vertex quorum. We claim the byzantine detector has eventual accuracy. Because without more information, it can not decide which part of its' quorum is byzantine nodes. But as we'll see. Eventually it will get the minimal vertex quorum which contains only correct nodes.

The node broadcast the suspicion to the minimal vertex quorum and the nodes inside the sink component will execute a consensus to decide which suspicious party is byzantine. The correct nodes will vote for the correct nodes and the byzantine nodes can vote arbitrarily. Since the quorum availability property holds for minimal quorums, we will get a quorum that only vote for the correct nodes and return.

\clearpage
\section{Group Membership In Resilient DB}

How to generalize group membership in dissemination quorum system?

Let $\{\mathit{C}_1, \mathit{C}_2, ..., \mathit{C}_z\}$ be a system. The membership that should be known by each process which is not the primary in the cluster are: local cluster members, the primary of all the other clusters and the corresponding members in the other clusters. The membership information should be known by the primary are local cluster members, all the primaries for other clusters and f+1 members for all the other clusters. For example, if we have two clusters: $\{\mathit{C}_1, \mathit{C}_2\}, \mathit{C}_1 = \{p_1, p_2, p_3, p_4\}, \mathit{C}_2 = \{q_1, q_2, q_3, q_4\}$. Let's suppose that $p_1, q_1$ are primaries in their corresponding clusters. Then membership function $\mathit{M}$ will return the following result: $\mathit{V}(p_1) = \{p_1, p_2, p_3, p_4, q_1, q_2\}, \mathit{V}(p_i) = \{p_1, p_2, p_3, p_4, q_1, q_i\}$, $ i = 2, 3, 4$. For processes in cluster 2, the results are symmetric.

At any point in time, the view of a process $p$ is denoted by $V(p)^x$, where $x$ is a unique numeric view identifier. In the initial view $x=0, \forall p \in \mathit{C}_i$ and $p$ is correct, then $\mathit{V}(p)^0 = \mathit{C}_i \cup \mathit{P} \cup \mathit{E}$, where $\mathit{P}$ is the set containing all the primary processes in each cluster and $\mathit{E}$ are extra information that is different for primaries and non-primary processes. For primary processes of the cluster $\mathit{E} = \cup_{\forall \mathit{C_i}, f+1 \textit{members of } C_i}$. For non-leader processes, $\mathit{E} = \{ \textit{one process from each cluster}\}$. Then within each cluster, the members have the same view about their local cluster members and the primary processes set. $\forall p \in \mathit{C}_i$, they agree on $\mathit{C}_i \cup P$. We denote the three components of $p$'s view $x$ as $C_p^x, P_p^x$ and $E_p^x$ respectively. 

$\mathbf{Uniqueness}$: If $p_i$ and $p_j$ are correct, $p_i, p_i \in \mathit{C_k}$ and  $V(p_i)^x$, $V(p_j)^x$ are defined, then $V(p_i)^x \setminus \mathit{E}_i^x = V(p_j)^x \setminus \mathit{E}_j^x$

$\mathbf{Validity}$: If $p_i$ is correct and $V(p_i)^x$ is defined, then $p_i \in V(p_i)^x$ and for all correct $p_j \in V(p_i)^x, V(p_j)^x$ is eventually defined.

$\mathbf{Integrity}$: If $p_i \in V(p_j)^x - V(p_j)^{(x+1)}$, then $\textit{Fail}(p_i)$ held at some correct process $p_j \in V(p_j)^x$, and if $p_i \in V(p_j)^{x+1} - V(p_j)^x$, then $\textit{Correct}(p_i)$ held at some correct $p_j \in V(p_j)^x$.

$\mathbf{Liveness}$: If there is a correct $p_i \in C_k$ such that $2f + 1$ correct members of $C_k$ do not suspect $p_i$ faulty, and  a $p_j \in C_k$ such that $\textit{Fail}(p_j)$ holds at $f + 1$ correct members of $C_k$, then eventually $C^{x+1}(p_i)$ is defined.

The uniqueness property states that correct processes in the same cluster share the same view over local cluster members and global primary processes.

Validity property states that correct process should be a member of its own view. Moreover, the correct members of its view will eventually aware of their membership.

Note that in the secure group membership paper, uniqueness and validity together imply that the correct process with defined $x$th views form a group. However, this is not the case in our definition. In Resilient DB, the uniqueness and validity together imply that the correct process in the same cluster share the same view information except the $E_i^x$ part.

Integrity property prevents byzantine processes changing the membership information arbitrarily. The failure or new member has to be detected by at least one correct process.

The liveness property prevents Byzantine processes from stalling the system forever. The condition can be interpreted as if the cluster is equipped with a eventual leader election module ($p_i$ is the leader) and the failure of some process ($p_j$) is detected by at least one correct process, then a new view will be installed driven by the correct leader($p_i$).


The protocol:

The purpose of the protocol is to ensure the processes in the same cluster keeps a consistent view on $V(p_i)^x \setminus E(p_i)^x$ and $V(p_j)^x \setminus E(p_j)^x$, which means the local cluster members and global primary processes should be the same for processes within one cluster. Here we denote this consistent partial view as $V(C_k)^x$ for each cluster. Then $V(C_k)^{x+1}$ is obtained by the members of $C_k$ either adopting the manager's suggestion and updating the group membership accordingly or removing the manager from the group. 

Correct manager:

The protocol structure when the manager is correct is very similar to PBFT. 


==> TradeOffExtra.tex <==

☞{Relation of responsiveness (strong validity of reconfiguration) of Byzantine failure detector}


\begin{theorem}[]
	\label{thm:theorem-impl2}
	There is no $\mathsf{Add}$ 
% 	and $\mathsf{join}$
	reconfiguration protocol that is
	consistency-preserving,
	availability-preserving,
	and responsive.
\end{theorem}

\xl{We have not used policy in the proof. This is more like a proof for validity: a reconfiguration protocol can not preserves consistency and availability at the same time and be responsive.}

% ——————————————
% Summary of Trade-offs

% Leave
%    P
%    A
%    R
% ——————
% Theorem? C P R
% Theorem? C A R
% ——————
% % % % % 
% Protocol 1
% C P     A X
% Protocol 2
% C A     P X


% ——————————————
% Add:
%  Theorem. Not have:
%    P
%    A
%    R
% —————
% Theorem 1.
%    C 
%    A
%    R
% —————
% Theorem 2.
%    C
%    SP    
%    R
% % % % % % % % % 
% 9.X
%   C P      A X                 SP weakened
% 9
%   C A      P X    SP X      In contrast to 1

% ——————————————


% \begin{theorem}[]
% 	\label{thm:theorem-impl2p}
% 	There is no $\mathsf{Add}$ 
% % 	and $\mathsf{join}$
% 	reconfiguration protocol that is
% 	consistency-preserving,
% 	strict policy-preserving, 
% 	and responsive.
% \end{theorem}


\begin{proof}
% The proof is by contradiction for each protocol:
% 
% The $\mathsf{add(q)}$ operation:
% 
Consider the quorum system $𝓠$ 
% (that we saw \autoref{thm:theorem-impl} and \autoref{fig:impl-example})
that we see in \autoref{fig:impl-example}
with four processes $𝓟 = \{1, 2, 3 \}$ and their individual minimal quorums: 
$𝓠(1)$ $=$ $\{\{1, 3 \}\}$, 
$𝓠(2)$ $=$ $\{\{2, 3\}\}$, 
and
$𝓠(3)$ $=$ $\{\{2, 3\}, \{1, 3\}\}$.
% $𝓠(4)$ $=$ $\{\{1, 3, 4\}\}$.
We will consider two scenarios based on whether the process $1$ is Byzantine.
In both, the processes $2$ and $3$ are well-behaved, and 
the process $2$ requests to $\mathsf{Add}$ a new quorum $\{1, 2\}$.
First, consider that the process $1$ is well-behaved.
% all the processes are well-behaved, 
The quorum system $𝓠$ is 
both consistent and available for $\{1, 2, 3 \}$.
% and available for $\{1, 2, 3, 4\}$.
% 
If process $2$ requests to add a new quorum $\{1, 2\}$, 
all processes still enjoy consistency and availability. 
Therefore, the $\mathsf{Add}$ operation is enabled. 
Since the protocol is assumed to be responsive, 
the process $2$ will eventually have $\{1, 2\}$ in its individual minimal quorums.
% 
Now, let us consider the scenario where the process $1$ is Byzantine.
% 
The quorum system
$𝓠$ is 
both consistent and available for $\{ 2, 3\}$.
% consistent for $\{ 2, 3, 4 \}$,
% and available for $\{ 2, 3 \}$.
% 
No process (including processes $3$) can distinguish whether process $1$ is Byzantine or not.
% 
Therefore, 
% it still approves the leave request from the process $2$.
the process $2$ still eventually add $\{1, 2\}$ as its individual minimal quorum,
and result in the updated quorum system $𝓠'$. 
% 
%Before the add quorum operation from $2$,
%the quorum $\{2, 3\}$ made $3$ available.
The quorum $\{1, 2\}$ for $2$,
and the quorum $\{1, 3\}$ for $3$
intersect at the Byzantine process $1$.
Therefore, to preserve consistency,
either 
$3$ should be added to $\{1, 2\}$ or 
$2$ should be added to $\{1, 3\}$.
% 
In both cases, the other quorum for that process is $\{2, 3\}$
which is a subset of the new quorum $\{1, 2, 3\}$.
% 
However, this violates the definition of individual minimal quorums.
Therefore, the quorum $\{2, 3\}$ needs to be dropped.
However, then the availability of processes $2, 3$ is violated
since their only other quorum $\{1, 2, 3\}$ contains the Byzantine process $1$.

% We consider two cases:
% First, 
% if the protocol does not change the individual minimal quorums of other well-behaved processes, 
% $𝓠'$ is only consistent for $\{3, 4\}$, which is a strict subset of $\{2, 3, 4\}$.
% % the well-behaved processes $𝓦' = \{2, 3, 4\}$.
% Therefore, consistency-preservation is violated.
% % 
% ☞{Removing $\{ 1, 3, 4 \}$ leaves no quorums, Add $2$ to it, violates policies. But adding should be fine (?)}
% Second,
% if the protocol changes the individual minimal quorums of other well-behaved processes as follow: 
% $𝓠'(3)$ $=$ $\{\{ 2, 3 \}\}$, 
% $𝓠'(4)$ $=$ $\{\{ 1, 2, 3, 4 \}\}$, 
% then policy-preservation is violated.
% Notice that if we add $\{1, 2, 3, 4\}$ into process $3$'s quorum system, since $\{2, 3\}$ is a strict subset of $\{1, 2, 3, 4\}$ and is a individual minimal quorum of process $3$, $\{1, 2, 3, 4\}$ is automatically ignored.
% There are some other possible individual minimal quorums for process $3$ and $4$ which keep consistency for the new quorum $\{1, 2\}$. 
% But they all require process $3, 4$ to change individual minimal quorums and violate their policies.

\end{proof}


==> Xtras.tex <==
8. There is no cycle composed only from one-direction edges in the sink component.

8. There is no one-direction edge in the sink component: $\forall p, q \in \mathbf{Sink}$, if $(p, q) \in E$, then $(q, p) \in E$. We can prove this statement by contradiction in all the cases. Let's assume that there is a one direction edge in the sink component: $\exists p, q, \in \mathbf{Sink}$, such that $(p, q) \in E \land (q, p) \notin E$. 

The first case is that there are only two vertices in the sink component. We reach a contradiction. Because the sink component is strongly connected. But there is no path from $q$ to $p$. 

The second case is that there are only three vertices in the sink component. Then we have $(p, q) \in E \land (q, r) \in E \land (r, p) \in E$ because of the existence of one path from $q$ to $p$ with $(q, p) \notin E$. $\{ q \} \notin \mathbf{MQ}$ becasue of $(q, r) \in E$. The same goes for $\{ r\} \notin \mathbf{MQ} \land \{ p \} \notin \mathbf{MQ}$. From statement 5 we have the minimal quorums are in the sink component. Then the minimal quorums contains as least two vertices. From statement 1, we know that minimal quorums are cliques. Then we can only have minimal quorums as $\mathbf{MQ} = \{ \{q, r\}, \{r p\} \}, \mathbf{MQ} = \{ \{q, r\} \} or \mathbf{MQ} = \{ \{r p\} \}$. Without losing of generality, let's assume that $ \{q, r\} \in \mathbf{MQ}$. 
%Then we have $(p, r) \in E$ because of statement 2. 
Since all the quorums contains at least one minimal quorum, we have $\{p, q, r\} \in \mathbf{MVQ}(p)$. Then for vertex $r$, we can have $\{r, p\} \in \mathbf{MVQ}(r)$ or $\{q, r, p\} \in \mathbf{MVQ}(r)$. If $\{r, p\} \in \mathbf{MVQ}(r)$, then we have $\{r, p\} \in \mathbf{MQ}$, which contradict $\{p, q, r\} \in \mathbf{MVQ}(p)$. If $\{q, r, p\} \in \mathbf{MVQ}(r)$, it contradicts with $\{q, r\} \in \mathbf{MQ}$.
%it will contradict $\{p, q, r\} \in \mathbf{MVQ}(p)$

The last case is when there are more than three vertices in the sink component. Because we have $(p, q) \in E \land (q, p) \notin E$ and the sink component is strongly connected. Then there is a path from $q$ to $p$. Let's assume that the last vertex in the path is $s$ and we have $(s, p) \in E$. Because $(p, q) \in E \land (q, p) \notin E$, we have $\exists Q_1 \in \mathbf{MVQ}(p) \land p, q \in Q_1$. And because the edge from $p$ to $q$ is one-direction, we have $\exists Q_3 \subset Q_1 \land p \notin Q_3 \land Q_3 \in \mathbf{MVQ}(q) \land (p, r) \in E$. For vertex $s$, we have $\exists Q_2 \in \mathbf{MVQ}(s) \land p, s \in Q_2$. From quorum intersection property, we have $Q_2 \cap Q_3 \notin \emptyset$. Then we have $\exists r \in Q_2 \cap Q_3, $

How to reduce more than three vertices to the case of three vertices.

One sink in the byzantine quorum graph is the necessary condition for a correct corresponding  byzantine quorum system.

%First of all, the sink component itself is a quorum in the system. Notice that not all strongly connected component is a quorum in the system. The strongly connected component with outgoing edges may not be able to form a complete quorum. Secondly, every quorum in the system contains at least one minimal quorum. If the minimal quorums (top-tires) are not completely inside the sink component, $\exists T \in \Q, T \nsubseteq Sink$, then for all the processes outside of the sink components $ \forall t, t \in T \setminus Sink, \exists s \in Sink, (t, s) \in E, (s, t) \notin E $. This contradicts the statement that minimal quorums are strongly connected subgraphs.

%Statement: the quorum intersection with at least one correct process condition = the sink component after the removal of byzantine processes is still strongly connected. 

This necessary condition can be checked when a process suspect some processes and try to remove them from its own quorums without losing safety property.  

%We prove the equivalence in two directions. 

We prove that the quorum intersection with at least one correct process implies the minimal quorum set is still strongly connected. 

%the sink component after the removal of byzantine process is still strongly connected. $\forall U_1, U_2 \in \mathbf{U}, \forall B \in \mathbf{B}, U_1 \cap U_2 \notin B \implies \forall B \in \mathbf{B}, (Sink \setminus B, E \setminus B )$ is strongly connected. We prove this statement by contradiction. Let's assume that $\exists B \in \mathbf{B}, (Sink \setminus B, E \setminus B)$ is not strongly connected. 

%Then there will be at least two disjoint components and that will produce disjoint minimal quorums, which violates the assumption. 

Maybe useful to add and remove processes while maintaining safety.

The sink component is like the leader?

What does the strongly connected component means? Is it a subset of minimal vertex quorum?

What is the relation between minimal vertex quorums and quorums? The quorum system constructed from minimal vertex quorums with quorum intersection and quorum availability is the necessary and sufficient condition for the original quorum system to hold the same properties.

Necessity: We want to prove that: with a fixed actual Byzantine failure set $B$, we have $\forall Q_1 \in \Q(v), \forall Q_2 \in \Q(v'), Q_1 \cap Q_2 \setminus B \neq \emptyset \wedge \exists v'',  Q_3 \in \Q(v''), Q'' \cap B = \emptyset$, then we can infer $\forall v, v'', \forall Q_1 \in MVQ(v), \forall Q_2 \in MVQ(v'), Q_1 \cap Q_2 \setminus B \neq \emptyset \wedge \exists v'',  Q_3 \in MVQ(v''), Q'' \cap B = \emptyset$. The proof for quorum intersection is straightforward. All the minimal vertex quorums are quorums for some specific nodes, we can directly apply the quorum intersection property for quorums to get the quorum intersection property for minimal vertex quorums. For quorum availability, if we have $ \exists v'',  Q_3 \in \Q(v''), Q'' \cap B = \emptyset$, then acoording to the definition of minimal vertex quorum, either $Q_3 \in MVQ(v'')$ or $\exists Q_4 \subset Q_3, Q_4 \in MVQ(v'')$. Either way there exists a minimal vertex quorum of node $v''$ that does not overlap with $B$. 


==> impossibility.tex <==
% ☞{This is broadcast, Stellar consensus is essentially broadcast}

\begin{definition}[Availability]
	\label{def:available}
	A quorum system 
	$𝓠$ 
	is available
	for a well-behaved subset of processes $P$
	iff
	every process in $P$ has at least a quorum that is well-behaved and quorum including:
	$∀ p ∈ P \subseteq \W, ∃ q ∈ 𝓠(p) \wedge q ⊆ P$, such that $∀ p' ∈ q, ∃ q' ∈ 𝓠(p'), q' ⊆ q$.
\end{definition}

\textbf{Necessary Conditions}

In this section, we consider the necessary conditions of a heterogeneous quorum system for consensus protocols.

A consensus protocol is expected to satisfy the following properties.

\begin{definition}[Specification of Consensus] \ 
% Consider a set of processes $P$.
\label{def:agreement-within-s}	
\label{def:validity-within-s-C}
\label{def:termination}
\begin{itemize}
    \item 
    (Agreement).
    No two well-behaved processes decide differently.	

    \item 
    (Strong validity).
    If all well-behaved processes propose the same value $v$, 
	then no well-behaved process decides 
% 	a value different from $v$;
	a different value;
	otherwise, a well-behaved process may only decide a value that was proposed by some well-behaved process or a special fixed value.
	
	\item 
	(Weak validity).
	If all processes are well-behaved and propose the same value $v$, 
	then no well-behaved process decides 
	% 	a value different from $v$;
	a value different from $v$;
	furthermore, if all processes are well-behaved and some process decide a value $v$, 
	then that value $v$ was proposed by some process.
	
   % \item 
    %(Termination for set $P$).
    %Every well-behaved process in $P$ eventually decides.
    
\end{itemize}
\end{definition}

For liveness, we define it to be very weak compared to normal termination property, which makes our conclusion more general.
Normally termination requires every well-behaved process eventually decides.
However, our quorum-based definition only requires that there exists an execution where only a quorum of $p$ take steps and then $p$ deceides.
(The same as FLP liveness. They do not require every admissible run to be a deciding run. The existence of a deciding admissible run is enough) 

% \begin{definition}[Agreement for set $P$]
% 	\label{def:agreement-within-s}	
% 	No two well-behaved processes in $P$ decide differently.
% \end{definition}
% 
% % \begin{definition}
% % 	\label{def:validity-within-s-RB}
% % 	Validity for reliable broadcast within set $S$: 
% % 	If the sender process is correct and broadcasts a value $v$, 
% % 	then every well-behaved process in $S$ eventually delivers $v$.
% % \end{definition}
% 
% \begin{definition}[Validity for set $P$]
% 	\label{def:validity-within-s-C}
% 	If all well-behaved processes propose the same value $v$, 
% 	the no well-behaved process in $P$ decides a value different from $v$;
% 	otherwise, a well-behaved process in $P$ may only decide a value that was proposed by some well-behaved process or a special preset value.
% \end{definition}
% 
% % \begin{definition}
% % 	\label{def:totality-within-s}
% % 	Totality for set $P$: 
% % 	If a well-behaved process in $P$ decides a value, 
% % 	then every well-behaved process in $P$ eventually decides a value.
% % \end{definition}
% 
% \begin{definition}[Termination for set $P$]
% 	\label{def:termination}	
% 	Every well-behaved process in $P$ eventually decides.	
% \end{definition}


% Liveness:
% Every member of $P$ eventually decides a value.
% ($P$ is a subset of well-behaved)


% \begin{definition}
% 	\label{def:extened-totality}
% 	Extended totality for $S$: 
% 	If a well-behaved process $p₁$ delivers / decides a value,
% 	then every well-behaved process $p₂ ∈ S$ eventually delivers /decides a value.
% \end{definition}


% \begin{definition}[Quorum-based reliable broadcast]
% 	\label{def:quorum-based-rb}
% 
% 	(1) Necessity of a quorum:
% 	If a well-behaved process $p$ delivers a message, 
% 	then there must be a quorum $q$ of $p$ such that $p$ has received at least one message from each member of $q$.
% 	
% % 	2. Well-behaved process's states are only defined by the states and messages of its own quorum members. \xl{can be integrated with 3?}
% 	
% 	(2) Sufficiency of a quorum:
% 	If $q$ is a quorum of a participant $p$, $p ∈ 𝓦$, and 
% 	the (well-behaved?) sender broadcasts $v$, 
% 	then there exists an execution in which {∗only $p$ and members of $q$} take steps and $p$ eventually delivers $v$.
% 
% \end{definition}

\newpageprime

We now state the properties of quorum-based protocols.

\begin{definition}[Quorum-based Consensus Protocol \cite{losa2019stellar}] \ 
\label{def:quorum-based-consensus}
\begin{itemize}
    \item 	
	(Safety). 
	If a well-behaved process $p$ decides, 
	then there must be a quorum $q$ of $p$ such that 
	$p$ receives at least one message from each member of $q$.

	\item
	(Sufficency of quorum)
	A well-behaved process $p$ can only observe the state of its quorum members.

    \item
    (Liveness). 
	If $q$ is a quorum of a well-behaved process $p$,
% 	and $v$ is a proposal value, 
% 	and $v$ is a proposal value, 
% 	in $q$,
	then there exists an execution in which only $p$ and members of $q$ take steps, 
% 	and $p$ eventually decides $v$.
	and $p$ eventually decides.
	
	\xl{There is a quorum $q$ of an available process $p$, such that there is an execution in which only $p$ and members of $q$ take steps and $p$ eventually decides. (This is the liveness for intact and consensus cluster)}

\end{itemize}
\end{definition}

\xl{If we want the normal liveness, any quorum can push decision, then every quorum needs to have inclusion.}

Our proofs apply for information-theoretic setting, where Byzantine processes have unlimited computation resource and is able to simulate any correct process's behavior.
Notice that our proof will break if a public key infrastructure is accessible for all the processes.
In another word, we assume that a process can verify the sender of a message.
However, it has no way to verify the sender of forwarded messages.
In our HQS setting, if $q$ is a quorum of process $p$, then the messages sent by $p'$, which is a member of $q$, can be verified by $p$.
But any forwarded messages from $p'$ to $p$ can not be verified by $p$.

%\newpageprime

% ☞{Revise, state the lemma}

The necessity of consistency and weak availability
% of the quorum system
was noted in 
previous work \cite{losa2019stellar}.
No quorum-based protocol can provide agreement for well-behaved processes
if the quorum system is not consistent.
% 
No quorum-based protocol can provide termination for processes $P$ of a quorum system
if the quorum system is not weakly available for $P$.


% \newpageprime

% lemma 4
% presented a lemma.
% shows that the necessary condition for consensus's agreement property is the well-behaved intersection between any pairs of quorums of well-behaved processes.

% However, their lemma 7 is only the necessary condition for the validity part of liveness property. 
% The same lemma here:
% 
% \begin{lemma}
% 	\label{lem:quorum-based-validity}
% % 	No quorum-based protocol can provide validity 
% % 	for a process which does not have at least one well-behaved quorum.
% % 	
% % 	A quorum-based protocol can provide validity for processes $P$ of a quorum system
% % % 	A quorum system has
% % 	only if
% % 	the quorum system is weakly available for $P$.
% 
% 	No quorum-based protocol can provide termination for processes $P$ of a quorum system
% % 	A quorum system has
% 	if
% 	the quorum system is not weakly available for $P$.
% \end{lemma}
% 
% \begin{proof}
% Consider a quorum-based protocol that provides termination for a well-behaved process $p$.
% % We assume there exists a quorum based protocol that provides validity to a well-behaved process $p$.
% % which does not have at least one well-behaved quorum.
% Consider an execution where Byzantine processes remain inactive.
% By the termination property,
% the process $p$ eventually decides.
% % if a correct sender broadcasts a value, 
% % $p$ delivers a value. 
% By the definition of quorum-based protocols,
% $p$ has received a message from each member of one of its quorums.
% Therefore, $p$ has a well-behaved quorum.
% % which contradicts the assumption.
% % that $p$ does not have a well-behaved quorum.
% \end{proof}

\begin{comment}
	When $S$ is not a quorum closure, we have $∃ p ∈ S, ∀ q ∈ 𝓠(p), q \nsubseteq S$ 
	Assume that the correct sender broadcast value $a$. By validity property, all the processes in $S$ deliver $a$. 
	We select an execution where
	$𝓟 ∖ S$ are Byzantine and remain silent.
	Before $p ∈ S$ delivers $a$, by the definition of quorum based algorithm, $p$ receives messages from one of its quorums $q$. Since Byzantine processes are slient, the messages are from $S$ and $q ⊆ S$, which contradicts 
	the assumption that $p$'s quorums are not included in $S$.
\end{comment}

\newpageprime

We now show that quorum inclusion is necessary for quorum based consensus protocols with weak validity.

\begin{lemma}
	\label{lem:quorum-based-totality}
	No deterministic quorum-based consensus protocol
	can provide agreement and weak validity for a quorum system, 
% 	if there is a process in $P$ that does not have at least one quorum $q$ that is well-behaved and quorum including.
    if the quorum system is not available.
% 	if there is a process in $P$ that does not have at least one quorum $q$ that is well-behaved and quorum including.
% 	for $q$.
\end{lemma}

%\xl{We require global agreement. Validity and termination are limited to $P$.}

\begin{proof}

Availability is a combination of weak availability and quorum inlusion property. 
We focus on the quourm inclusion property for now.

We construct the proof by contradiction.
First we assume there is a quorum-based algorithm that provides all the properties for consensus without quorum inclusion.
Then by a sequence of indistinguishable executions, we reach to a contradiction of the desired properties.
% The proof is contradiction.
%We consider quorum systems that are not available for $P$,
% for a set of well-behaved processes $P$,
%and
%show that any quorum-based protocol violates either validity or termination for $P$.
% for a set $P$.
% We assume that there is a protocol that can provide validity and termination for a set $P$.
% Let $p$ be a well-behaved process in $P$.
%   

We define initial configurations as an array of values that each process proposes.
For simplicity, we consider binary proposals, either $0$ or $1$.
We use $\bot$ to represent Byzantine processes' proposal. 
Byzantine processses are free to change their proposals and the validity does not dependent on their inputs.
% (including a Byzantine proposal).
% that Byzantine processes can propose any value and behave arbitrarily.

We define admissible execution where the Byzantine processes in the execution do not exceed the maximum Byzantine set $\B$.
Since the Byzantine consensus's properties are defined for correct processes, the maximum Byzantine set $\B$ for a quorum system $\Q$ is a set of the failures can be tolerated at the same time in $Q$ while satisfying all the properties of consensus.

Consider a quorum system $\Q$ for processes $\P = \{1,$ $2,$ $3 \}$.
The quorum system is defined as $\Q(1) = \{\{1, 3\}\}$, $\Q(2) = \{\{1, 2\}\}$, $\Q(3) = \{\{2, 3\}\}$.
Assume there is a quorum-based algorithm that can provide consensus without quorum inclusion.
Then for $\Q$, $\B = \{\{1\}, \{2\}, \{3\}\}$.
Since any single Byzantine process will leave the remaining quorums with proper intersections and at least a quorum weakly available without Byzantine process.

1. We define $C_1 = \langle 0, 0, 1 \rangle$, $C_2 = \langle 0, 0, 0 \rangle$, $C_3 = \langle 0, 0, \bot \rangle$, $C_4 = \langle \bot, 0, 1 \rangle$. 
Without further clarification, a configuration without $\bot$ as initial input is considered to have all the processes well-behaved.
We construct $E_1$ in $C_1$ where only process $\{2, 3 \}$ take steps. 
By quorum's liveness, process $3$ eventually decides. 
By weak validity and all the processes are correct, process $3$ decides a value proposed by some process. 
Without loss of generality, we assume process $3$ decides $1$.
We construct $E_2$ in $C_2$ where only processes in $ \{1, 3\}$ take steps. 
By quorum's liveness, process $1$ eventually decides. 
By weak validity and all the processes are correct and propose $0$, processes $1$ decides $0$.
We construct $E_3$ in $C_3$ where at first Byzantine process replay $E_1$ with correct process $2$ and then replay $E_2$ with correct process $1$. 
Then Byzantine process $3$ stops taking steps. By the liveness of the quorum system, correct process $2$ eventually decides. 
By agreement and correct process $1$ decides $0$, process $2$ decides $0$.
We construct the final execution in $C_4$. 
We let processes in  $\{2, 3\}$ replay $E_1$ first and correct process $3$ decides $1$. 
Then Byzantine process $1$ fakes its state as after the replay of $E_2$. 
Since correct process $2$ can not distinguish this final execution with the previous one, it replay $E_3$ and decides $0$. 
Thus agreement is violated. 
Two correct processes decide different values. 

2. We define $C_1 = \langle 0, 0, 0 \rangle$, $C_2 = \langle 1, 1, 1 \rangle$, $C_3 = \langle 0, 1, \bot \rangle$, $C_4 = \langle \bot, 1, 1 \rangle$. 
Without further clarification, a configuration without $\bot$ as initial input is considered to have all the processes well-behaved.
We construct $E_1$ in $C_1$ where only process $\{1, 3 \}$ take steps. 
By quorum's liveness, process $1$ eventually decides. 
By weak validity and all the processes are correct and propose $0$, process $1$ decides $0$.
We construct $E_2$ in $C_2$ where only processes in $ \{2, 3\}$ take steps. 
By quorum's liveness, process $3$ eventually decides. 
By weak validity and all the processes are correct and propose $1$, processes $3$ decides $1$.
We construct $E_3$ in $C_3$ where at first Byzantine process replay $E_2$ with correct process $2$ and then replay $E_1$ with correct process $1$. 
Then Byzantine process $3$ stops taking steps. 
By the liveness of the quorum system, correct process $2$ eventually decides. 
By agreement and correct process $1$ decides $0$, process $2$ decides $0$.
We construct the final execution in $C_4$. 
We let processes in  $\{2, 3\}$ replay $E_2$ first and correct process $3$ decides $1$. 
Then Byzantine process $1$ fakes its state as after the replay of $E_2$. 
Since correct process $2$ can not distinguish this final execution with the previous one, it replay $E_3$ and decides $0$. 
Thus agreement is violated. 
Two correct processes decide different values. 
\xl{This construction does not need the second part of weak validity.}

In both $E_3$ and the final execution, the Byzantine process exhibit Byzantine behavior by sending conflicting messages or changing their proposal.

If quorum inclusion is provided this proof will break.
There are two cases that quorum inclusion can be provided.

1. All the processes have the same quorum $\{1, 2, 3\}$. 
In this case, $\B = \emptyset$ and $E_3$ and the final execution are not admissible executions.

2. Process $1$ includes additional quorum $\{1, 2\}$ in tis quorum system. 
Then the quorum $\{1, 2\}$ has inclusion. 
However, $\B = \{\{3\}\}$ and the final execution is not admissible execution. 
Since Byzantine process $1$ is not tolerated by the quorum system $\Q$.

Note that including more quorums to have inclusion will break the quorum intersection and will not enlarge the maximum Byzantine set. 
For example, if we have the quorum system as $\Q'(1) = \{\{1, 3\}, \{1 , 2\}\}$, $\Q'(2) = \{\{1, 2\}\}$, $\Q'(3) = \{\{2, 3\}, \{1, 3\}\}$. 
Then the corresponding $\B = \{\{3\}\}$ and is still the same.
If we have the quorum system as $\Q''(1) = \{\{1, 3\}, \{1 , 2\}\}$, $\Q'(2) = \{\{1, 2\}, \{2, 3\}\}$, $\Q'(3) = \{\{2, 3\}\}$. 
Then the corresponding $\B = \{\{1\}\}$ and still does not tolerate the last two executions.
If we have the quorum system as $\Q''(1) = \{\{1, 3\}, \{1 , 2\}\}$, $\Q'(2) = \{\{1, 2\}, \{2, 3\}\}$, $\Q'(3) = \{\{2, 3\}, \{1, 3\}\}$. 
Then the corresponding $\B = \emptyset$.

\textbf{Generalization}

%Our proof can generalize to any quorum system $\Q$ with at least two processes that do not have quorum inclusion.
%Assume that $p_1, p_2$ are the two processes without quorum inclusion.
%Let $q_1$ be $p_1$'s quorum and $q_2$ be $p_2$'s quorum.
%Since $p_2$ does not have quorum inclusion, then there is a $p_3$ that all its quorum is not completely inside $q_2$.
%Let one of $p_3$'s quorum be $q_3$.
 
 Now consider the general case.
 Partition the quorum system into three sets $S_1$, $S_2$ and $S_3$.
 For all the processes in $S_1$, we let their quorums be $S_1 \cup S_2$.
 For all the processes in $S_2$, we let their quorums be $S_2 \cup S_3$.
 For all the processes in $S_3$, we let their quorums be $S_1 \cup S_3$.
 In this quorum system, any one of the three sets can be Byzantine and the quorum system still has quorum intersection and weak availability.
 We let the processes in $S_1$ run the consensus just as process $1$ in our previous example.
 Processes in $S_2$ run consensus as process $2$ and  Processes in $S_3$ run consensus as process $3$.
 Then by the same construction, we arrive at the conclusion that no quorum based algorithm can provide consensus for this quorum system.

\textbf{Sufficency Proof}



\begin{comment}
	Let $P = \{1, 3\}$.
	% $𝓠₁$ is not available for $P$ since their quorums are not quorum including.
	% does not have at least one well-behaved quorum with inclusion for well-behaved processes in $P$.
	% 
	Consider the initial configuration $[0, 0, 0]$ for $\Q_1$.
	Consider the execution $E_0$ 
	where the messages between processes except those between process $1$ and $2$ are delayed.
	By validity, only $0$ can be decided.
	By the liveness of quorum-based protocol, process $2$ delivers $0$.
	
	Consider 
	%another 
	another initial configuration 
	% $C_1 =$ 
	$[0, 0, 1]$ for $\Q_1$.
	%We delay the messages between process $1$ to the rest of the system until process $2$ decide $1$, which is the same as $E_1$.
	We replay the excution $E_0$. 
	Since the initial states of processes $1, 2$ does not change, process $2$ decides $0$.
	By termination, process $3$ eventually decides.
	By global agreement, process $3$ decides $0$, too.
	We define this execution to be $E_1$.
	By the sufficency of quorum (\xl{or liveness of quorums?}), $E_1$ can be an execution with only processes $2, 3$ taking steps. 
	
	%Consider the execution $E₁$ 
	%where the messages between processes except those between process $1$ and $2$ are delayed.
	% by termination for $P$ (\autoref{def:termination}) and 
	%By the liveness 
	% property 
	%of quorum-based protocols,
	% (\autoref{def:quorum-based-consensus}),
	%and agreement for $P$ (\autoref{def:agreement-within-s}), $1$ eventually decide $1$.
	%Let the execution after $2$'s decision and before $1$'s decision be $E_2$.
	% there exists an execution $E_1$ that 
	%the process $2$ can decide $0$.
	%☞{Why? Is liveness too strong?}
	% with only $\{1, 2\}$ taking steps.
	%Since $1$'s quorum is $\{1, 2\}$,  then by the definition 2 of quorum-based algorithm (\autoref{def:quorum-based-consensus}), $E_2$ can be an excution with only $1$ and $2$ are the participants.
	
	
	%Consider a initial configuration $C_1 = [1, 1, 1, 1]$ for $Q_1$.
	%By validty of consensus (\autoref{def:validity-within-s-C}) and the quorum-based consensus definition (\autoref{def:quorum-based-consensus}), there exists an execution $E_1$ where only process $2$ and its quorum members $\{2, 3, 4\}$ take step and $2$ eventually decides $1$. 
	
	
	Consider a quorum system $𝓠₂$ that is the same as $𝓠₁$ 
	except that the process $2$ is Byzantine. 
	% Consider a similar quorum system $\Q_2$ for processes $\P = \{1, 2, 3, 4\}$ where only the process $2$ is Byzantine.
	% The quorums are defined as $\Q_2(1) = \{\{1, 2\}\}$, $\Q_2(2) = \_$, $\Q_2(3) = \_$, $\Q_2(4) = \{\{1, 3, 4\}\}$.
	% Notice that the quorums for well-behaved processes are the same in $𝓠₁$ and $𝓠₂$.
	We note that $𝓠₂$ is not available for $P$.
	Since process $1$'s quorum is weakly available but does not satisfy quorum inclusion
	and process $3$'s quorum is not weakly available.
	%since their quorums are not well-behaved (\ie, not weakly available).
	☞{Shouldn't $P$ be well-behaved?}
	☞{Isn't 1 befouled? Can't we have an example where instead of weak availability, inclusion is not satisfied?}
	%\xl{no inclusion}
	% ☞{because not have weak availability}
	% does not have at least one well-behaved quorum with inclusion for well-behaved process in $P$.
	% 
	Consider a initial configuration 
	% $C_2 =$ 
	$[1, 0, 1]$ for $𝓠₂$.
	Since all the well-behaved processes propose $1$,
	by the validity property of consensus, 
	only $1$ can be decided.
	% 
	Consider the execution $E₂$ where
	the Byzantine process $2$ replays its execution in $E_1$.
	%If the process $3$ does not decide, termination is violated.
	The well-behave process $3$ cannot distinguish between the two configurations $[0, 0, 1]$ and $[1, 0, 1]$ based on the state of its quorum members $\{2, 3\}$.
	Therefore, since the consensus algorithm is deterministic, process $3$ decides $0$, which violates validity.
	It is the same case for process $1$.
	Process $1$ can decides $0$ by agreement for set $P$ and violates validity.
	Or it never decides and violates termination for set $P$.
	% The process $1$ cannot distinguish between $E₁$ and $E₂$ based on the state of its quorum $\{1, 2\}$.
	% Therefore, either the process $1$ does not decide, which violates termination,
	% or
	% deterministically decides $1$, which contradicts with validity.
\end{comment}
\end{proof}

%In the example, process $1$ is weakly available in both quorum systems $Q_1$ and $Q_2$. 
%However, it does not enjoy availability because of violation of quorum inclusion.
%Adding inclusion for process $1$ will break the construction of th example above.
%$E_1$ and $E_2$ are distinguishable

\textbf{Impossibility for Byzantine Reliable Broadcast}

\begin{definition}[Specification of Reliable Broadcast] \ 
		\label{def:agreement-rb}	
		\label{def:validity-rb}
		\begin{itemize}
			\item 
			(Consistency).
			No two well-behaved processes deliver different values.	
			
			\item 
			(Validity).
			If a correct process $p$ broadcast a message $m$, then every correct process that is available eventually delivers $m$.
			
			 \item 
			(Totality for quorum-based algorithms).
			If some message is delivered by any correct process, there exists an execution for the available process $p$ where only quorum a $q$ of $p$ take steps and eventually $p$ delivers a message.
			
			\item
			(No duplication)
			Every correct process delivers at most one message.
			
			\item
			(Integrity)
			If some correct process delivers a mesage $m$ with sender $p$ and process $p$ is correct, then $m$ was previously broadcast by $p$.
			
		\end{itemize}
\end{definition}

\begin{proof}
	The proof is similar to consensus.
	The difference between reliable broadcast and consensus is on the validity and totality (termination).
	For reliable broadcast, there is a sender who broadcasts a value and we do not need to provide any validity gurantee when the sender is Byzantine.
	We define the initial configuration as values received by the processes from the sender.
	Without further clarification, a configuration without $\bot$ as initial input is considered to have all the processes well-behaved, including the sender.
	For reliable broadcast, we
	We define $C_1 = \langle 0, 0, 0 \rangle$, $C_2 = \langle 1, 1, 1 \rangle$, $C_3 = \langle 0, 1, \bot \rangle$, $C_4 = \langle \bot, 1, 1 \rangle$. 
	We construct $E_1$ in $C_1$ where only process $\{1, 3 \}$ take steps. 
	By quorum's liveness, process $1$ eventually delivers a value. 
	By validity and the correct sender broadcasts $0$, process $1$ delivers $0$.
	We construct $E_2$ in $C_2$ where only processes in $ \{2, 3\}$ take steps. 
	By quorum's liveness, process $3$ eventually delivers a value. 
	By validity and the correct sender broadcasts $1$, processes $3$ delivers $1$.
	We construct $E_3$ in $C_3$ where the sender is Byzantine.
	At first Byzantine process $3$ and the sender replay $E_2$ with correct process $2$ and then replay $E_1$ with correct process $1$. 
	Then Byzantine process $3$ stops taking steps. 
	By the totality for quorum-based algorithm and the liveness of the quorum system, correct process $2$ eventually delivers a value. 
	By consistency and correct process $1$ delivers $0$, process $2$ delivers $0$.
	We construct the final execution in $C_4$ where the sender is Byzantine. 
	We let processes in  $\{2, 3\}$ replay $E_2$ first and correct process $3$ delivers $1$. 
	Then Byzantine process $1$ fakes its state as after the replay of $E_2$. 
	Since correct process $2$ can not distinguish this final execution with the previous one, it replay $E_3$ and delivers $0$. 
	Thus consistency is violated. 
	Two correct processes deliver different values. 
\end{proof}

\begin{comment}

\newpageprime

% We proved that no protocol can provide validity, termination within $S$ when the well-behaved process $p \in S$ does not have at least one well-behaved quorum with inclusion.

We prove stellar protocol is sufficient to provide validity, totality and agreement for $S$ when the quorum system have quorum intersection and well-behaved process in $S$ has at least one well-behaved quorum with inclusion in $S$.

proposition 12: Given a set of faulty processes, all the processes in $S$ are not blocked by $\P \setminus (S \cup \B)$.

lemma 16: if well-behaved process in an execution send messages Ready(a) and Ready(a'), then a = a'. (don't need proposition 9)

Proof sketch for agreement within $S$ does not change.

lemma 38 and lemma 17 can be translated to: Any well-behaved process's quorum is blocking for well-behaved process in $S$: $\forall p \in \P, \forall q \in \Q(p), q \cap \W$ is blocking $\forall p' \in S \cap \W$.
Proof sketch for totality: then all the well-behaved processes in $S$ will send Ready messages.
Eventually, the well-behaved quorum inside $S$ will push every well-behaved process to deliver.

Proof sketch for validity: When sender is correct, all the well-behaved processes sends echo message with $v$ to all the processes in the system.
Eventually the well-behaved quorums in $S$ will deliver the echo message and send Ready message.
Then the well-behaved processes in $S$ deliver $v$.

\end{comment}


\begin{comment}
	% Totality
	% Agreement
	
	As an example, consider 
	two quorum system $𝓠$ and $𝓠'$
	for processes $𝓟 = \{ 0, 1, 2, 3, 4 \}$.
	% where the byzantine processes are $\{ 3 \}$ and 
	% well-behaved processes are $𝓦 = \{1, 2, 4\}$,
	In $𝓠$ and $𝓠'$, the processes $0$ is well-behaved and Byzantine respectively.
	In both $𝓠$ and $𝓠'$
	the process $3$ is Byzantine,
	and
	the processes $1$, $2$, $4$ are well-behaved.
	% 
	The quorum of $0$ is arbitrary in $𝓠$.
	In both $𝓠$ and $𝓠'$,
	the quorums for $1$, $2$ and $4$ are
	% $𝓠(1) = \{\{1, 2, 3\}\}$, 
	$\{\{1, 2, 3\}\}$, 
	% $𝓠(2) = \{2, 3, 4\}$,
	$\{2, 3, 4\}$,
	and
	% $𝓠(4) = \{1, 3, 4\}$.
	$\{1, 3, 4\}$.
	% and the quorums for $0$ are unspecified. 
	
	
	We construct two executions $E$ and $E'$ in $𝓠'$
	that are indistinguishable for $1$ 
	but the process $1$ decides $v₀$ and $v₁$ respectively.
	% 
	We construct $E$ through a sequence of transformations for executions $E₀$, $E₁$ and $E$.
	In the execution $E$,
	the process $0$ sends $v₀$.
	By validity, the process $4$ will eventually deliver $v₀$.
	
	
	
	We only define initial configurations on well-behaved processes since Byzantine sender and processes are able to behave arbitrarily. 
	% 
	We define two initial configurations corresponding to the value that the sender sends to each process.
	$\langle 1, 2, \_, 4\rangle$:
	$C₁ = \langle 0, 1, \_, 0 \rangle$, 
	$C₂ = \langle 0, 1, \_, 1 \rangle$. 
	% 
	The Byzantine process $3$ behaves as a correct process that received value $0$ for process $4$ in the first configuration. 
	% 
	In the second configuration, it behaves as a correct process received value $1$ to process $2$. 
	% 
	According to \autoref{def:quorum-based-algorithm}, 
	$C₁$ is a deciding run for value $0$ 
	and 
	$C₂$ is a deciding run for value $1$:
	In $C₁$, $4$ delivers $0$ and then all the well-behaved processes deliver $0$; 
	In $C₂$, $2$ delivers $1$ and then all the well-behaved processes deliver $1$. 
	However, in process $1$'s view, the well-behaved members of its quorum have the same initial configuration in $C₁$ and $C₂$. Then whether to deliver $0$ or $1$ depends on the Byzantine process $3$. So $C₁ | 𝓠(1) = C₂ | 𝓠(1)$ and it is bivalent. 
	Since the exact Byzantine processes are unknown, we can apply the techniques in FLP paper and construct a bivalent run for process $1$ to violate totality property.  
	
	
	\begin{lemma}
		\label{lem:quorum-based-totality}
		A deterministic quorum-based protocol can provide totality and agreement
		% 	for a well-behaved process 
		for a process 
		only if
		it has at least one quorum that is 
		% 	well-behaved and 
		quorum including.
	\end{lemma}
	
	%By the assumption that processes in $S$ do not have at least one self-closed quorum in $S$, we have $∀ p ∈ S, ∀ q ∈ 𝓠(p) \wedge q ∈ S, ∃ p' ∈ q, ∀ q' ∈ 𝓠(p'), q' \nsubseteq q$. 
	
	%We construct an execution with a Byzantine sender $s$. $s$ sends brodcast $v₁$ to $q$ and cuts the communication outside $q$.
	%Then by the deifnition of quorum based algorithm 2, $p$ delivers $v₁$. By totality definition \autoref{def:termination}, $p'$ eventually delivers $v₁$. $p'$ can only deliver $v₁$ even without receiving all messages from its quorum.
	%We let the Byzantine sender broadcasts $v₂$ to other processes in $S ∖ q$. Since $B$ is unknown in the system, we let Byzantine processes sends the $v₂$ messages the same as those convinced $p'$ to deliver $v₁$. Then $p'$ delivers $v₂$ and violates consistency.  
	
	\begin{proof}
		Consider a well-behaved process $p$ that
		it does not any quorum that is 
		% well-behaved and 
		quorum including.
		We show that no protocol can provide totality for $p$.
		
		
		% Example: We construct an execution of federated Bracha protocol where either totality or consistency is violated in a non-self-closed quorum. Assume $𝓟 = \{1, 2, 3\}, 𝓦 = \{1, 2, 3\}, 𝓠(1) = \{\{1, 2\}\}, 𝓠(2) = \{\{2, 3\}\}, 𝓠(3) = \{\{1, 3\}\}$. We let the sender be Byzantine and sends broadcast $v$ message to process $1, 2$. Since process $1$ and $2$ can not distinguish Byzantine process and well-behaved process, the same messages can be from a correct sender. Then by the deinition 3 of quorum-based algorithm, there exists an execution where only processes $\{1, 2\}$ take steps and $1$ delivers $v$. By Bracha protocol, process $1, 2$ sends echo $v$ messages to $𝓟$. Since $\{1, 2\}$ is a quorum of process $1$, it sends ready $v$ messages to $𝓟$. However, process $2$ can not send ready $v$ message. Since $1$ is not blocking or a quorum of $2$. Then process $1$ can not deliver $v$ and contardict the assumption.
		% If process $1$ delivers $v$ after receive a quorum of echo messages, then totality might be violated. After process $1$ delivers, we let the Byzatine sender sends broadcast $v'$ message to $3$. Then well-behaved processes $2, 3$ receives contradicting messages and can not deliver $v$, which contradicts the assumption that we ensure totality property.
		
		
		% Consider a quorum $q$ of $p$ that is either not well-behaved or not quorum including.
		Consider a quorum $q$ of $p$ that is not quorum including.
		
		
		
		
		
		FLP proof process:
		
		Each process is modeled as a automaton. The configuration of the system contains the message buffer and internal state of each process which includes input register and output register. The initial configuration of the system contains an empty message buffer and the value assigned to the input register, which indicate the value received from sender.
		The input register can also be undefined since a Byzantine sender may choose to be silient for some processes.
		The output registers are not defined in the initial configuration. It can be written at most once with the delivered value from broadcast protocol.
		
		To simpify the problem, we limit the sender to brodcast only 0 or 1. Note that Byzantine sender can send different value to different processes and  even nothing to some processes in the initial configuration.
		
	\end{proof}
	
	
	\newpageprime
	Lemma 1:
	Suppose that from some configuration $C | q$, the schedule $\sigma₁, \sigma₂$ lead to configuration $C₁, C₂$ respectively. If the set of processes taking steps in $\sigma₁$ and $\sigma₂$ are disjoint for process $p$, then $\sigma₂$ can be applied to $C₁$ and $\sigma₁$ can be applied to $C₂$ and both lead to the same configuration $C_3 | q$.
	
	Commutative property of schedules:
	We define the commutative property in the Byzantine setting with a new definition of disjoint schedules.
	Two schedules are disjoint for a process $p$ if and only if the well-behaved processes in $p$'s quorums do not intersect: $(\sigma₁ | \cup 𝓠(p) ∩ 𝓦) ∩ (\sigma₂ | \cup 𝓠(p) ∩ 𝓦) = \emptyset$. 
	The intuition behind is that Byzantine processes can behave arbitrarily and we do not define their states. And based on the definition of quorum based algorithms, the state of a process is only defined by its quorum members' states and messages.
	
	In our example, $\sigma₁ | \{1, 2\} = \{1, 3, 4\} | \{1, 2\} = \{1\}, \sigma₂ | \{1, 2\} = \{2, 3, 4\} | \{1, 2\} = \{2\}$. Then $\sigma₁$ and $\sigma₂$ are disjoint schedules for process $1$.
	%In $\sigma₁$, it is possible that process $1$ only receives echo(0) from itself.
	%In $\sigma₂$, it is possible that process $1$ receives echo(1) and ready(1) messages from process $2$.
	%No matter the order of these messages, they lead process $1$ to the same state.
	
	We assume there is a quorum based algorithm P that implements Byzantine reliable broadcast.
	
	\newpageprime
	
	
	Lemma 2:
	
	P has a bivalent initial configuration for some well-behaved process. (we fix the value broadcast to be 1 or 0, then the initial configuration can be 1-valent, 0-valent and bivalent for a process. 
	Note that for a broadcast algorithm, when the sender is Byzantine, there is no guarantee for termination (bivalent is acceptable). 
	However, when the sender is correct, validity enforce the delivery of message (1-valent or 0-valent is the only correct schedule).)
	
	
	We prove by contradiction. Assume there is no bivalent execution for $p$. There are 0-valent and 1-valent initial configurations since correct sender can broadcast 0 or 1. 
	Then we find two adjacent initial configurations that $C_0$ is 0-valent and $C₁$ is 1-valent. 
	We assume that there is at least three well-behaved processes in the system. 
	The quorums are always self-closed for quorum systems with only one or two well-behaved processes,which contradicts our assumption that algorithm P implements Byzantine reliable broadcast for a process without well-behaved self closed quorums.
	We select the quorum of another process $p_0$ to include all the well-behaved processes with value 0 as initial input in $C_0$ and vice versa for $p₁$, 1 and $C₁$. 
	Then we set the quorum of $p$ to exclude the well-behaved process whose initial values are different in $C_0$ and $C₁$. 
	In this way we construct a quorum system without self-closure.
	Then in $C_0$, 0 will be delivered by $p_0$ and by totality $p$ will eventually deliver $0$. It is the same situation for $C₁$ and $p₁$. We prove contradiction by showing that the same initial configuration for $p$ leads to bivalent result.
	
	The example we showed above is a bivalent initial configuration for process $1$.
	
	\newpageprime
	Lemma 3: 
	
	Let $C | q$ be a bivalent configuration of $p ⃰$, and let $e = (p, m)$ be an event that is applicable in C. Let $\mathcal{E}$ be a set of configurations reachable from $C$ without applying $e$, and let $\mathcal{D} = \{e(E) | E ∈ \mathcal{E} \ \text{and e is applicable to E} \}$ Then $\mathcal{D} | q$ contains a bivalent cofiguration for $p ⃰$.
	
	We prove by contradiction. Assume that $\mathcal{D} | q$ contains no bivalent configuration for $p ⃰$. 
	%Let $E_i ∈ \mathcal{E}$ be an $i$-valent configuration reachable from $C$ and $i = 0, 1$. Let
	There exists two neighbors configurations $C_0, C₁ ∈ \mathcal{E}$ such that $D_i = e(C_i)$ is i-valent. Without loss of generality, $C₁ = e'(C_0), e'  =(p', m')$.
	Note that we only consider $p, p' ∈ q, q ∈ Q(p ⃰)$.
	
	Case 1: If $p' \neq p$, then $D₁ = e'(D_0)$ by lemma 1. This is impossible, since any successor of a 0-valent configuration is 0-valent.
	
	In our example, we let $C_0$ be the same after process $2$ receives $E(0)$ from process $4$. Let $e$ be the event when $1 $ receives $E(0)$ from $1$. Let $e'$ be the event when $2$ receives $R(0)$ from $4$. Then the resulting states are the same despite the order.
	
	Case 2: If $p' = p$, then consider any finite deciding run from $C_0$ in which $p$ takes no step or $p$ is Byzantine.
	
	Let $\sigma$ be the corresponding schedule, and let $A = \sigma(C_0)$. By lemma 1, $\sigma$ is applicable to $D_i$. If $p$ is well-behaved but takes not step in $\sigma$, then $\sigma$ is commutative with $e, e'$. If $p$ is Byzantine, then both $e$ and $e'$ are steps taken by Byzantine process and they commute with any schedule.
	Let $E_i = \sigma(D_i), i = 0, 1$.
	By lemma 1, $e(A) = E_0$ and $e(e'(A)) = E₁$. Since $D_0, D₁$ are univalent, their successors $E_0, E₁$ are univalent, too. Then $A$ is bivalent, which contradicts the assumption that $A$ is a deciding schedule.
	
	We seperate consistency and avaliablity requirements for quorum systems. A process can have avalability but not consistency as the example from instantiate paper:
	$𝓟 = \{1, 2, 3\}, 𝓦 = \{1, 2, 3\}, 𝓠(1) = \{\{1\}\}, 𝓠(2) = \{\{1, 2\}, \{2, 3\}\}, 𝓠(3) = \{\{1, 3\}, \{2, 3\}\}$. Then process $1$ is not consistent with process $2, 3$.
	A process can have consistency but not avalability:
	$𝓟 = \{1, 2, 3\}, 𝓦 = \{1, 2\}, 𝓠(1) = \{\{1, 2\}\}, 𝓠(2) = \{\{2, 3\}\}$.
	Process $2$ is consistent with other well-behaved process but does not have availability.
	
	
	
	% the following two properties:
	% % (Consensus cluster). A subset S ⊆ W of the well-behaved processs is a consensus cluster when:
	% \begin{itemize}
		% \item
		% Quorum Intersection:
		% % (safety):
		% % S is intertwined.
		% % The intersection of every pair of quorums is non-empty.
		% Every pair of quorums have an intersection.
		% % intersect.
		% \item
		% Quorum Availability:
		% % (liveness):
		% % If p ∈ S then there is a quorum Qp of p such that Qp ⊆ S.
		% Every process is a member of at least one quorum.
		% \end{itemize}
	
	
	% A quorum system $𝓠$ is a set of quorums with the following two properties:
	% % (Consensus cluster). A subset S ⊆ W of the well-behaved processs is a consensus cluster when:
	% \begin{itemize}
		% \item
		% Quorum Intersection (safety):
		% % S is intertwined.
		% % The intersection of every pair of quorums is non-empty.
		% Every pair of quorums have an intersection.
		% % intersect.
		% \item
		% Quorum Availability (liveness):
		% % If p ∈ S then there is a quorum Qp of p such that Qp ⊆ S.
		% Every process is a member of at least one quorum.
		% \end{itemize}
	
	%Note: Byzantine consistent broadcast does not require totality. Then the existence of a non-empty quorum closure is enough. But Byzantine reliable broadcast enforce totality, then a non-empty self-closed quorum is enforced to implement BRB. 
	
	\ \\
	\ \\
	
	☞{Find another word for individual quorum?}
	
	☞{Should we replace minimal with elementary? The instantiation paper used it.}
	
	☞{We have necessary conditions. Are they sufficient?}
	
	☞{
		The intersection should be in Intact to get totality like the opodis paper.
		The disc paper does not have totality, it is in W.
	}
	
\end{comment}

\textbf{Sufficency Proof}

We use a modified Bracha protocol to show that the necessary condition is also sufficent for Byzantine reliable broadcast.

The sender broadcasts a message $m$ to all the processes.
Upon receving $m$, correct processes echo this messsage among its followers.
%quorum members.
When a correct process receives a quorum of consistent echo messages $m$, it sends ready messages to all its followers. 
%quorum members.
A correct process can also send ready message with a different value from its echo message.
It sends the ready message when it receives consistent ready messages from a blocking set.
When a correct process receives a quorum of consistent ready messages $m$, it delivers $m$ and finishes the reliable broadcast.
 
 We prove that this algorithm provides Byzantine reliable broadcast when the quorum system satisfies our necessary condition: the quorum system is consistent and available.
 
\begin{proof} \
	
	\textbf{Consistency}
	
	A well-behaved process only delivers a message when it receives a quorum of consistency echo messages.
	If $p_1$ delivers $m_1$ with $q_1$ and $p_2$ delivers $m_2$ with $q_2$, then the correct process in $q_1 \cap q_2$ only sends ready messages with one value then $m_1 = m_2$.
	%Because our quorum system has at least a well-behaved process in the intersection of any pair of quourms.
	
	\textbf{Validity}
	
	When a correct sender broadcasts a messaeg $m$, the correct process $p$ that is available has a quorum $q$ that only has well-behaved members.
	They all echo the same message $m$ to their followers, including process $p$.
	Then process $p$ has a quorum of consistent echo message for $m$.
	Since availability requires every process $p' \in q$ has a quorum $q' \subseteq q$.
	By the same reasoning, $p'$ receives a quorum ($q'$) of consistent echo message for $m$.
	Then all the processes in $q$ send out ready messages to their followers.
	Process $p$ now has a quorum of consistent ready message and it delivers $m$.
	
	\textbf{Totality}
	
	A correct process delivers a  message $m$ when it receives a quorum $q$ of ready message for $m$.
	By the quorum intersection, $q$ intersects with all the quorums in the system at at least one well-behaved process.
	Then for any correct process $p'$, $q \cap \W$ is blocking: 
	$\forall p' \in \W, \forall q' \in \Q(p'), q \cap q' \cap \W \neq \emptyset$.
	Let's assume that $p_i$ is the well-behaved process in the correct intersection.
	Since $p_i \in q'$, $p'$ is $p_i$'s follower. 
	All the correct processes in $q$ send ready messages to their followers, including $p'$.
	Then $p'$ receives a blocking set of ready messages and starts sending ready messages to its followers.
	For an available process $p''$, it has a quorum that all the memebrs are well-behaved.
	Then $p''$ will receive the ready message from the quorum and deliver $m$.
	
	\textbf{No duplication}
	
	Since all the correct processes only sends out ready message for one $m$, every correct process can only collect at most one quorum of consistent ready message and deliver $m$ once.
	
	\textbf{Integrity}
	
	We prove that at least a quorum of echo messages was received for $m$ before the delivery.
	If a correct process delivers a message $m$, $m$ appears in a quorum $q_r$ of ready messages.
	By assumption, there is a non-empty set of available processes.
	Let process $p$ be available with its quorum $q$  and $q$ is well-behaved and quorum-inclusive.
	Then by quorum intersection, $q \cap q_r \neq \emptyset$.
	Let $p_i \in q \cap q_r$ which sents the ready message for $m$.
	$m$ can only be sent by a correct process in a ready message after a quorum of echo messages received for $m$ or a blocking set of ready messages received for $m$.
	If it's the first case, we complete the proof.
	If it's the second case, we prove that $p_i$ is not blocked by Byzantine processes and the first ready message sent by the process in $q$ is from a quorum of echo messages.
	Let the blocking set be $b$.
	By the quorum inclusion, $\exists q_i \in \Q(p_i), q_i \subseteq q \subseteq \W \wedge b \cap q_i \neq \emptyset$.
	Since $b$ always includes a process in $q$, by induction, the first process in $q$ which sends a ready message is triggered by receiving a quorum of echo messages.
	And we complete our proof.
	%Let $p_{i'} \in b \cap q_i$.
	%There is a correct process
	
	%Then the first ready message for $m$ is sent by receiving a quorum of echo messages for $m$.
	Every quorum of a well-behaved process includes well-behaved process.
	Then the echo message is sent by the correct processs after receiving it from the sender. 
	If the sender is correct, $m$ was previously broadcast by it.
	
\end{proof}


==> introduction_end.tex <==
In summary, this paper makes the following contributions.
\begin{slimitemize}
% \begin{itemize}[leftmargin=*]
		% \noindent
		% \begin{slimitemize}
% 			\item
% 			Measurements for the feasibility of reconfiguration attacks
% 			(\autoref{sec:reconfig-attack})
			
			\item
			A general model of heterogeneous quorum systems
			(\autoref{sec:q-systems}),
% 			\item 
			and
			their consistency, availability and inclusion properties.
% 			of heterogeneous quorum systems
			(\autoref{sec:prop-q-sys}).

			\item
			A graph characterization of heterogeneous quorum systems,
			and
			its application to 
			optimize reconfiguration			
			(\autoref{sec:graph-and-sink}),
			and
			% \xl{personal quorum system?}
			a sink discovery protocol
			% reconfiguration optimization
        (in the appendix \autoref{sec:discovery}).
%     and \autoref{sec:discovery}).
			
			% \item 
			% Necessary properties for heterogeneous quorum systems
			% to solve consensus
			% (\autoref{sec:necess-prop})
			
			\item 
			% Impossibilities and 
			Trade-offs between reconfiguration guarantees 
			(\autoref{sec:trade-off}).
			
			\item
			Reconfiguration protocols
			for joining and leaving of a process,
			and adding and removing of a quorum,
			and their proofs of correctness
			% (\autoref{sec:join} - \autoref{sec:add})
			(\autoref{sec:join},
			\autoref{sec:leave-and-remove-avail-pres},
			\autoref{sec:leave-remove-policy-pres},
			and
			\autoref{sec:add}).
% 			Join is straightforward and presented in the appendix \autoref{sec:join}).
      The proofs of the theorems are available in the appendix.

% 		\end{itemize}
		\end{slimitemize}
% 	

